A Dataset for Multi-intensity Continuous Human Activity Recognition through Passive Sensing

Human activity recognition (HAR) is essential in healthcare, elder care, security, and human-computer interaction. The use of precise sensor data to identify activities passively and continuously makes HAR accessible and ubiquitous. Specifically, millimeter wave (mmWave) radar is promising for passive and continuous HAR due to its ability to penetrate non-metallic materials and provide high-resolution wireless sensing. Although mmWave sensors are effective at capturing macro-scale activities, like exercising, they fail to capture micro-scale activities, such as typing. In this paper, we introduce mmDoppler, a novel dataset that utilizes off-the-shelf (COTS) mmWave radar in order to capture both macro and micro-scale human movements using a machine-learning driven signal processing pipeline. The dataset includes seven subjects performing 19 distinct activities and employs adaptive doppler resolution to enhance activity recognition. By adjusting the radar's doppler resolution based on the activity type, our system captures subtle movements more precisely. mmDoppler includes range-doppler heatmaps, offering detailed motion dynamics, with data collected in a controlled environment with single as well as multiple subjects performing activities simultaneously. The dataset aims to bridge the gap in HAR systems by providing a more comprehensive and detailed resource for improving the robustness and accuracy of mmWave radar activity recognition.

==> tex/Intro_back.tex <==
\section{Introduction}
Human activity recognition (HAR) is vital in fields such as healthcare, elder care, security, and human-computer interaction, relying on accurate sensor data to identify various activities. In this context, millimeter wave (mmWave) radar has emerged as a promising technology due to its ability to penetrate non-metallic materials, resilience to environmental changes, and high-resolution sensing capabilities. While traditional HAR methods use pointcloud data from sensors like LiDAR or depth cameras and effectively capture macro-scale activities such as walking or running where heavy body movements are involved~\cite{alam2020lamar, singh2019radhar, palipana2021pantomime,alam2021palmar}, they often struggle with micro-scale activities like typing or subtle hand movements. This limitation highlights the need to collect human activity datasets using advanced sensing mechanisms and deep learning counterparts to capture both macro and micro-scale human movements comprehensively.

This paper introduces a novel dataset of human activities collected using a Commercial off-the-shelf (COTS) mmWave radar designed to bridge the gap between macro and micro-scale activity recognition. Our dataset encompasses a broad range of activities, from macro-scale actions like walking and squats to micro-scale behaviours such as typing and sitting. The collection involves seven subjects performing 19 distinct activities in an indoor environment, providing a diverse and rich set of data for HAR research.

A key challenge when using mmWave radar for HAR is capturing the subtle movements associated with micro-scale activities. In order to address this issue, instead of capturing only the pointcloud dataset as done in the prior works~\cite{singh2019radhar, palipana2021pantomime, alam2020lamar}, we employ an innovative approach involving adaptive doppler resolution. Doppler resolution refers to the radar's ability to distinguish between different velocities of moving objects. Higher doppler resolution allows for more precise detection of small changes in movement, while lower doppler resolution is sufficient for detecting larger, more pronounced movements. By selecting an optimal doppler resolution based on the type of activity being performed, we can better capture the nuances of various movements.

A lower doppler resolution is used for macro-scale activities, characterized by greater movement (such as walking or running). This setting effectively captures the significant velocity changes associated with these activities without the need for fine detail. Conversely, a higher doppler resolution is employed for micro-scale activities involving minimal movement (such as typing or subtle hand gestures). This allows the radar to detect subtle velocity changes, providing a detailed and accurate representation of these activities. By using this adaptive doppler resolution approach, our system can robustly and precisely recognize a wide range of activities, even when subtle changes occur. This enhances the overall accuracy and versatility of HAR systems, making them more effective in various applications where both macro and micro-scale movements must be accurately captured.

Our dataset is generated using COTS IWR1642BOOST mmWave Radar. It captures the range-doppler heatmaps along with the traditional pointclouds for different human activities, where the range-doppler heatmaps is a 2D image representation where its abscissa is the range (where the human subjects are present), and the ordinate is the doppler speed at which the subjects are moving. These heatmaps combine range and doppler information from radar signals, offering a detailed view of motion dynamics over time. By leveraging range-doppler heatmaps, our dataset captures the intricate details of both large and small movements, enabling more accurate and nuanced activity recognition and mitigating the challenges of traditional pointcloud-based datasets.

In addition to the adaptive doppler resolution and range-doppler heatmaps, our dataset collection methodology includes the following key features:
\begin{itemize}
    \item \textbf{Diverse Activity Set:} We have included a wide array of 19 different activity classes from Activities of Daily Living (ADLs), Instrumental Activities of Daily Living (IADLs) [9], and daily indoor exercises – (i) macro activities like walking, running, jumping, clapping, lunges, squats, waving, vacuum cleaning, folding clothes, changing clothes, and (ii) micro activities like laptop-typing, phone-talking, phone-typing, sitting, playing guitar, eating food, combing hair, brushing teeth, and drinking water to ensure comprehensive coverage of daily human behaviours. 
    \item \textbf{Controlled Environment:} Data collection was conducted in a controlled indoor environment to minimize external noise and ensure the quality and consistency of the data. Our dataset comprises 75K frames of data, $5 \times$ greater than the state-of-the-art HAR mmWave dataset in existence~\cite{singh2019radhar}.
    \item \textbf{Multiple Subjects:} Our dataset uniquely includes multiple subjects performing various activities simultaneously, unlike traditional datasets that typically focus on single-subject activities~\cite{singh2019radhar, palipana2021pantomime, ahuja2021vid2doppler}. This feature allows our dataset to account for the complexity and variability of real-world scenarios where interactions between multiple individuals are common.
\end{itemize}

\swadhincomment{Please add more dataset info and its implications}
\swadhincomment{Please also add some related work in the intro}

\AS{Added.}

As a result, our dataset provides a valuable resource for researchers and developers working on HAR systems using mmWave radar. Combining adaptive doppler resolution and range-doppler heatmaps enables more accurate and robust activity recognition across a wide range of activities. By combining mmWave radar technology with point cloud data, this work overcomes the limitations of previous HAR systems based on point clouds. Making this dataset public will enable further research and development of innovative solutions that leverage the capabilities of mmWave radar to comprehensively and reliably detect human activity.
